Revisiting Image-Language Networks for Open-ended Phrase Detection

Most existing work that grounds natural language phrases in images starts with the assumption that the phrase in question is relevant to the image. In this paper we address a more realistic version of the natural language grounding task where we must both identify whether the phrase is relevant to an image and localize the phrase. This can also be viewed as a generalization of object detection to an open-ended vocabulary, introducing elements of few- and zero-shot detection. We propose an approach for this task that extends Faster R-CNN to relate image regions and phrases. By carefully initializing the classification layers of our network using canonical correlation analysis (CCA), we encourage a solution that is more discerning when reasoning between similar phrases, resulting in over double the performance compared to a naive adaptation on three popular phrase grounding datasets, Flickr30K Entities, ReferIt Game, and Visual Genome, with test-time phrase vocabulary sizes of 5K, 32K, and 159K, respectively.

==> sections/retrieval_experiments.tex <==
\subsection{Image-Sentence Retrieval Experiments}
To show that CCA is an effective way of aligning the image and text features on other tasks, we evaluate this approach on the task of image-sentence retrieval on the MSCOCO~\cite{lin2014microsoft} and Flickr30K~\cite{young2014image} datasets.  In this task the goal is to retrieve a relevant image when provided a descriptive sentence, or to retrieve a relevant sentence provided an image. It is typically evaluated using Recall@$K$ where $K$ = \{1, 5, 10\}.  We also report mean recall (mR), which averages the different recall thresholds.  We follow the experimental settings for the Embedding Network~\cite{wangTwoBranch2017} used in~\cite{burnsLanguage2019}.  More specifically, for the text representation we used the same HGLMM features used by our phrase detectors that are fine-tuned on the retrieval task (unlike phrase detection, where they are kept fixed since fine-tuning didn't improve performance significantly). We also used a 152-layer ResNet pretrained on ImageNet~\cite{deng2009imagenet} and averaged over ten crops that have been resized to 448x448 inputs for our image representation.

As seen in Table~\ref{tab:image-sentence}\footnote{Some methods have shown better performance than those we report by either fine-tuning the visual features~\cite{FaghriArxiv2017,Song_2019_CVPR}, or identifying regions that match to semantic concepts~\cite{huangArxiv2017,lee2018stacked}.  We only compare to methods using the same visual representation as our experiments.}, using CCA for layer initialization provides consistent gains on both datasets.  This demonstrates that using CCA for layer initialization can benefit tasks other than phrase detection.

\begin{table*}
\centering
\setlength{\tabcolsep}{3pt}
\caption{Image-sentence retrieval results on the MSCOCO 1K test set using a fixed 152-layer ResNet. (a) reports the state-of-the-art on this task and (b) compares the approach of Wang~\etal~\cite{wangTwoBranch2017} with and without CCA initialization using a modified version of their code.}
\label{tab:image-sentence}
\begin{tabular}{|rl|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\hline
& & \multicolumn{7}{|c|}{MSCOCO} & \multicolumn{7}{|c|}{Flickr30K} \\
\cline{3-16}
& & \multicolumn{3}{|c|}{Image-to-Sentence} & \multicolumn{3}{|c|}{Sentence-to-Image} & & \multicolumn{3}{|c|}{Image-to-Sentence} & \multicolumn{3}{|c|}{Sentence-to-Image} &\\
\cline{3-16}
& & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & mR & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & mR\\
\hline
\hline
\textbf{(a)} & \textbf{State-of-the-art} & & & & & & &\\
& RRF~\cite{Liu_2017_ICCVs}& 56.4 & 85.3 & 91.5 & 43.9 & 78.1 & 88.6 & 74.0 & 47.6 & 77.4 & 87.1 & 35.4 & 68.3 & 79.9 & 66.0\\
& VSE++~\cite{FaghriArxiv2017} & 58.3 & 86.1 & 93.3 & 43.6 & 77.6 & 87.8 & 74.5 & 43.7 & 71.9 & 82.1 & 32.3 & 60.9 & 72.1 & 60.5\\
& CMPM~\cite{Zhang_2018_ECCV} & 56.1 & 86.3 & 92.9 & 44.6 & 78.8 & 89.0 & 74.6 & 49.6 & 76.8 & 86.1 & 37.3 & 75.7 & 75.5 & 66.8\\
& Chain-VSE~\cite{Wehrmann_2018_CVPR} & 61.2 & 89.3 & 95.8 & 46.6 & 81.9 & 90.9 & 77.6 & -- & -- & -- & -- & -- & -- & --\\
& DAN~\cite{Nam_2017_CVPR} & -- & -- & -- & -- & -- & -- & -- & 55.0 & 81.8 & 89.0 & 39.4 & 69.2 & 79.1 & 68.9\\
\hline
\textbf{(b)} & Embedding Network~\cite{burnsLanguage2019} & 67.2 & 91.7 &\textbf{97.5} & 53.0 & 84.0 & 92.2 & 80.9 & 60.5 & 86.4 & \textbf{92.9} & 43.8 & 73.9 & 83.3 & 73.5\\
& Embedding Network w/CCA Initialization & \textbf{67.8} & \textbf{92.9} & 97.3 & \textbf{53.9} & \textbf{85.2} & \textbf{93.7} & \textbf{81.8} & \textbf{61.7} & \textbf{86.8} & \textbf{92.9} & \textbf{45.4} & \textbf{74.4} & \textbf{83.6} & \textbf{74.1}\\
\hline
\end{tabular}
\end{table*}

